The extended Ville's inequality for nonintegrable nonnegative supermartingales

Following the initial work by Robbins, we rigorously present an extended theory of nonnegative supermartingales, requiring neither integrability nor finiteness. In particular, we derive a key maximal inequality foreshadowed by Robbins, which we call the extended Ville's inequality, that strengthens the classical Ville's inequality (for integrable nonnegative supermartingales), and also applies to our nonintegrable setting. We derive an extension of the method of mixtures, which applies to $\sigma$-finite mixtures of our extended nonnegative supermartingales. We present some implications of our theory for sequential statistics, such as the use of improper mixtures (priors) in deriving nonparametric confidence sequences and (extended) e-processes.

==> ENSM/BCI-BvM.tex <==

\subsection{Credible intervals}

Recall a common object of Bayesian interest, the $(1-\alpha)$-credible interval  of the parameter $\theta$, which is a 
$(X_1,\dots, X_n)$-based interval $\hat I_n$ such that $ \pi_n(\hat I_n) \ge 1-\alpha$ (for any data; i.e.\ almost 
surely on data's probability space $\Omega$). We have the following frequentist-Bayesian link when $\pi_0$ is proper.

\begin{proposition} Suppose the prior $\pi_0$ is a probability measure \emph{that does not depend on $\theta$}.
    The $(1-\alpha)$-CS formed by Ville's inequality on the likelihood ratio mixtures $M_n^{\pi_0,\theta}$ at time $n$,
    \begin{equation}
        \CI_n =\{ \theta : M_n^{\pi_0,\theta} \le 1/\alpha \},
    \end{equation}
    is also a $(1-\alpha)$-credible interval.
\end{proposition}

\begin{proof}
    
Integrating the both sides of
\begin{equation}
    \frac{\d  \pi_n}{\d \pi_0}(\theta) = \frac{1}{M_n^{\pi_0,\theta}}
\end{equation}
over any (data-dependent) interval $J$, we have
\begin{equation}
  \pi_n(J) =  \int_J \frac{\d  \pi_n}{\d \pi_0}(\theta) \pi_0(\d \theta) = \int_J \frac{1}{M_n^{\pi_0,\theta}} \pi_0(\d \theta).
\end{equation}
Taking $J$ to be the complement of $\CI_n$, $J = \{ \theta : M_n^{\pi_0,\theta} > 1/\alpha \}$,
\begin{equation}
  \pi_n(J) =   \int_J \frac{1}{M_n^{\pi_0,\theta}} \pi_0(\d \theta) \le \int_J \alpha \pi_0(\d \theta) = \alpha \pi_0( J ) \le \alpha.
\end{equation}
Consequently, $\pi_n(\CI_n) \ge 1-\alpha$.
\end{proof}

We remark that the ``prior does not depend on $\theta$'' assumption is important as otherwise...


Let us look at the Bayesian Z-test example, where the family is $\normals_{\sigma^2 = 1}$. Consider $\pi_0 = \normal{0}{1}$
 as the prior. Then, with $X_1,\dots, X_n$ the observations, the posterior is
 \begin{equation}
     \pi_n = \normal{\frac{S_n}{1+n}}{\frac{1}{1+n}}.
 \end{equation}
Recall from \cref{sec:mix-n0c} that
\begin{equation}
   \CI_n =  \left[ \frac{S_n}{n} \pm \sqrt{ \frac{ \log \frac{1 + n}{\alpha^2}  + \frac{S_n^2}{n(1+n)} }{n} } \right]
\end{equation}
is the CS formed by the likelihood ratio mixtures $M_n^{\normal{0}{1},\mu}$. So the actual coverage is

\begin{equation}
    \pi_n(\CI_n) =  \normal{\frac{S_n}{1+n}}{\frac{1}{1+n}} \left\{  \left[ \frac{S_n}{n} \pm \sqrt{ \frac{ \log \frac{1 + n}{\alpha^2}  + \frac{S_n^2}{n(1+n)} }{n} } \right] \right\},
\end{equation}
which is experimentally seen to often be much more than $1-\alpha$. This means that the Ville-based CS as a credible interval is quite conservative. Nevertheless, the result above establishes an interesting link between these fundamental objects. 




\subsection{?? Bernstein-von Mises}
Recall that
\begin{equation}
  \frac{\pi_n(\theta)}{\pi_0(\theta)}  = \frac{1}{M_n^{\pi_0,\theta}}.
\end{equation}
If the posterior satisfies the BvM theorem,
\begin{equation}
    \int \left| n^{-1/2}  \pi_n(\hat\theta_n + n^{-1/2} \theta') - p_{0, 1/I(\hat\theta_n)}(\theta') \right| \d \theta' \to 0.
\end{equation}
One may hope that, \emph{pointwise},
\begin{equation}
     \pi_n( \theta)  \approx p_{\hat\theta_n, 1/(nI(\hat\theta_n))}(\theta), \quad M_n^{\pi_0,\theta} \approx \frac{ \pi_0(\theta) }{p_{\hat\theta_n, 1/(nI(\hat\theta_n))}(\theta) } = \frac{\sqrt{2\pi} \cdot \pi_0(\theta) \cdot \exp\{ n(\theta-\hat\theta_n)^2 I(\hat\theta_n) /2\} }{ \sqrt{nI(\hat\theta_n)}  }.
\end{equation}
Note that in the Gaussian prior and flat prior Z-test cases, the $\approx$ above holds with equality.
